Efficient Ensemble for Fine-tuning Language Models on Multiple Datasets

This paper develops an ensemble method for fine-tuning a language model to multiple datasets. Existing methods, such as quantized LoRA (QLoRA), are efficient when adapting to a single dataset. When training on multiple datasets of different tasks, a common setup in practice, it remains unclear how to design an efficient adaptation for fine-tuning language models. We propose to use an ensemble of multiple smaller adapters instead of a single adapter per task. We design an efficient algorithm that partitions $n$ datasets into $m$ groups, where $m$ is typically much smaller than $n$ in practice, and train one adapter for each group before taking a weighted combination to form the ensemble. The algorithm leverages a first-order approximation property of low-rank adaptation to quickly obtain the fine-tuning performances of dataset combinations since methods like LoRA stay close to the base model. Hence, we use the gradients of the base model to estimate its behavior during fine-tuning. Empirically, this approximation holds with less than $1\%$ error on models with up to $34$ billion parameters, leading to an estimation of true fine-tuning performances under $5\%$ error while speeding up computation compared to base fine-tuning by $105$ times. When applied to fine-tune Llama and GPT models on ten text classification tasks, our approach provides up to $10\%$ higher average test accuracy over QLoRA, with only $9\%$ more FLOPs. On a Llama model with $34$ billion parameters, an ensemble of QLoRA increases test accuracy by $3\%$ compared to QLoRA, with only $8\%$ more FLOPs.

==> influence.tex <==
\section{Efficiently Estimating Task-level Influence}

\HZ{could we think about how to implement this more efficiently as well}

Suppose there are $n$ tasks. Let us denote their data as $(X_1, Y_1)$, $(X_2, Y_2)$, $\dots$, $(X_n, Y_n)$.
When we train a model (like a foundation model) on all the combined data of the $n$ tasks, we use a loss function such as the one below:
\begin{align}
    \hat \cL(f_W) = \frac 1 n \sum_{i=1}^n \hat L(f_W(X_i), Y_i).
\end{align}
Above, we are using set-based notations to denote the loss of task $i$ as $\hat L(f_W(X_i), Y_i)$, which may be the sum of individual losses of each sample, or the average risk of the entire set.

Here, we are interested in understanding the effect of one task on the prediction of other tasks.
To formalize this, let us denote $\hat \theta$ as
\begin{align}
    \hat \theta \leftarrow \arg \min_{W} \hat \cL (f_W).\label{eq_hat_theta}
\end{align}
For a given task $i$, let us denote the minimizer without using task $i$ as $\hat \theta_{- i}$, defined as
\begin{align}
    \hat \theta_{- i} \leftarrow \arg \min_{W} \frac 1 {n-1} \sum_{j = 1:~j \neq i}^n \hat L(f_W(X_j), Y_j).\label{eq_hat_theta_i}
\end{align}
We may write $\hat \theta_{-i}$ equivalently as follows
\begin{align}
    \hat \theta_{- i} &\leftarrow \arg \min_W  \frac 1 {n-1} \left( n \hat \cL (f_W) - \hat L (f_W(X_i), Y_i) \right) \\
    &= \arg \min_W \hat \cL(f_W) - \frac 1 n \hat L (f_W(X_i), Y_i).
\end{align}

\emph{When the number of tasks $n$ is large}, the second term above is of order $O(n^{-1)}$ (assuming the loss value is bounded by a small constant).
Thus, one may estimate the difference in the perturbed parameters using an approximation technique.
Concretely, let us define
\begin{align}
    \hat \theta_{\epsilon, i} = \arg \min_W \left( \hat \cL(f_W) + \epsilon \hat L(f_W(X_i), Y_i) \right). \label{eq_theta_eps_i}
\end{align}
Denote $\Delta_{\epsilon} = \hat \theta_{\epsilon, i} - \hat \theta$ as the change of parameters.
Because $\hat \theta_{\epsilon, i}$ is a minimizer of equation \eqref{eq_theta_eps_i}, taking the gradient over $W$, we get a stationary point condition as
\begin{align}
    0 = \nabla \hat \cL(f_{\hat \theta_{\epsilon, i}}) + \epsilon \nabla \hat L(f_{\hat \theta_{\epsilon, i}}(X_i), Y_i).
\end{align}
We now perform Taylor's expansion of the above, around $\hat \theta$ (since when $\epsilon \rightarrow 0$, $\hat \theta_{\epsilon, i} \rightarrow \hat \theta$).
Dropping the second-order Taylor's expansion error term, we arrive at the following
\begin{align}
    0 \approx \nabla \hat \cL(f_{\hat \theta}) + \epsilon \nabla \hat L(f_{\hat \theta}(X_i), Y_i) + \left( \nabla^2_W \hat \cL(f_{\hat\theta}) + \epsilon \nabla_W^2 \hat L(f_{\hat\theta}(X_i), Y_i) \right) \Delta_{\epsilon}. \label{eq_delta_epsilon}
\end{align}
Since $\hat \theta$ is a minimizer of $\hat \cL(f_W)$ from equation \eqref{eq_hat_theta}, the gradient at this parameter is zero.
Thus, we may now simplify the above equation \eqref{eq_delta_epsilon} to solve $\Delta_{\epsilon}$ as:
\begin{align}
    \Delta_{\epsilon} = - \epsilon \left[ \nabla_W^2 \hat \cL(f_{\hat \theta})\right]^{-1} \nabla \hat L(f_{\hat \theta}(X_i), Y_i).
\end{align}
To conclude, we have now shown that
\begin{align}
    \hat \theta_{-i} = \hat \theta + \frac 1 n \left[ \nabla^2 \hat \cL(f_{\hat \theta}) \right]^{-1} \nabla \hat L(f_{\hat \theta}(X_i), Y_i),
\end{align}
assuming the loss function of each task is twice-differentiable.

\paragraph{Efficient algorithm:}
To calculate the above Hessian inverse product term, one may use the following relation:
\[ {H_{\hat \theta}}^{-1} v \leftarrow \arg \min_x \left(\frac 1 2 x^{\top} H_{\hat \theta} x - x^{\top} v  \right). \]
Here, we denote the Hessian matrix as $H$.
This is a quadratic minimization problem, which can be solved with fast iterative methods.


==> results.tex <==
\section{Detailed Description of the Approach}

\subsection{Clustering Algorithms}

\subsection{Mathematical Notations}\label{tab_notation}
We provide a list of symbols and their meaning used in the paper for reference below:
\begin{itemize}
    \item $S$: A subset of $\set{1, 2, \dots, n}$.
    \item $f_i(S)$: {The performance of a model fine-tuned on tasks in $S$, evaluated on task $i$}.
    \item $\theta^\star$: {The vectorized model weights of the pretrained initialization}.
    \item $\hat\theta_S$: {The vectorized model weights fine-tuned on a subset of tasks $S$}.
    \item $h_{\theta^\star}(s, y)$: Model loss given an input pair $s, y$.
    \item $\nabla h_{X}(s, y)$: {Vectorized gradients of model output with respect to model weights $X$}.
    \item $T_{i}$: {The average performance of $f(S)$ over multiple subsets $S$ that include task $i$}, for every $i = 1, 2, \dots, n$.
    \item $h^{(m)}(s, y)$: The ensemble model at iteration $m$, i.e., ensembling the first $m$ models built by a boosting approach. 
\end{itemize}

\subsection{Technical details}

\subsubsection{Clustering task relevance scores}


We now describe a clustering algorithm to partition the $n$ tasks into $k$ disjoint subsets.
Given an $n$ by $n$ task relevance score matrix $T$, we will find a clustering that maximizes the average density of all clusters.
Concretely, let $C_1, \dots, C_k$ be a disjoint partition of $[n]$. 
Let $v_1, \dots, v_k$ be a $0$-$1$ vector indicating whether a task is in one cluster or not.
The average density of this clustering can be written as:
\begin{align*}
   \frac 1 k \sum_{i=1}^{k} \frac{v_i^{\top} T v_i}{v_i^{\top} v_i}. \label{eq_obj} 
\end{align*}
This integral objective is NP-hard to optimize in general.

We design a Semi-Definite Programming (SDP) relaxation and then round the SDP solution to a clustering.
Let us denote the assignment variables as an $n \times k$ matrix $V$, such that each entry $V_{i,j}$ indicates whether a task $i$ belongs to a cluster $j$, for every $i = 1, \dots, n$, $j = 1, \dots, k$.
Moreover, let the $j$th column of $V$, which is the characteristic vector of the $j$-th cluster, be denoted as $v_j$.
Under this assignment, the sum of $V_{i, j}$ across any task $i$ must be one, as we allow one task to be assigned in a single group. By contrast, the sum of $V_{i, j}$ across $C_j$ is the number of tasks assigned to  $C_j$, which is at least one.

Let $e$ denote the all-ones vector. We state an integer program to maximize the average density of all $k$ clusters as follows
\begin{align*}
    \max_{V\in\real^{n\times k}}~~&  \BigInner{T}{ \frac 1 k\sum_{j=1}^k \frac{v_j v_j^{\top}}{v_j^{\top}v_j}} \nonumber \\
    & Ve = e, \sum_{i=1}^n V_{i,j} \geq 1 \text{ for } 1 \leq j \leq k \nonumber \\
    & V_{i, j} \in \set{0, 1}, \text { for any } 1 \le i\le n, 1 \le j\le k.
\end{align*}
Note that $v_iv_i^{\top}$ is a rank-one semidefinite matrix.
Let us denote the sum of them (normalized by $v_i^{\top}v_i$) as the following new variable
\begin{align*}
    X = \sum_{j=1}^k \frac{v_j v_j^{\top}}{v_j^{\top}v_j}.
\end{align*}
$X$ has rank $k$ since it is the sum of $k$ rank-$1$ matrices, and the $v_i$'s are orthogonal to each other. Additionally, its trace is equal to $k$ because the trace of $\frac{v_j v_j^{\top}}{v_j^{\top}v_j}$ is one for any $j$.
Second, one can verify that the entries of every row of ${X}$ sum up to one.
Removing the $0$-$1$ integer constraint, we derive a rank-constrained problem as
\begin{align*}
    \max_{X\in\real^{n\times n}}~~& \inner{T}{X} \\
        & X e = e, \tr[X] = k, \textup{rank}(X) = k \\
        & X \geq 0,  X \succeq 0.
\end{align*}
Further relaxing the rank constraint (while keeping the trace constraint) leads to a convex program, which can be solved efficiently.

Given a solution of the SDP, denoted as $\hat X$, the last step is to round $\hat X$ into an integer solution.
We set a threshold $\lambda$ such that if $\hat X_{u,v} \ge \lambda$, tasks $u$ and $v$ are assigned to the same cluster.
In the experiments, we set $\lambda$ as $c/n$ for a constant $c\ge 1$, since $\hat X_{u,v}$ should be $\frac{1}{|C_i|}$ when they are in the same cluster with $|C_i|< n$.
Thus, the intra-cluster distance must always be at least $\lambda$ with the assignment.


\subsubsection{AdaBoost} 
At each iteration, the sample weights are modified, and a new model is trained on the reweighted training samples. 
Denote the error rate of $h^{(m)}$ at iteration $m$ as $err^{(m)}$. 
Denote $\alpha^{(m)} = \log \frac{1 - err^{(m)}}{err^{(m)}}$. 
The training samples that are misclassified by the classifier $h_{\theta^{(m-1)}}$ have their weights increased exponentially by $err^{(m)}$.  
\[
w_i^{(m)}  \leftarrow w_i^{(m-1)} \exp\Big(\alpha^{(m)}\mathbb{1}\big(y_i \neq h_{\theta^{(m)}}(s_i, y_i)\big)\Big)
\]

In our implementation, weights are assigned to separate tasks, instead of single tasks. 
We use parameter-efficient fine-tuning to fit each model, such as LoRA and Adapters. 
At each iteration, a new model is fit on a reweighted version of the training dataset. Similarly, the first-order approximation can also be applied to this case, by solving a reweighted version of logistic regression on gradients. 
Therefore, we leverage Algorithm \ref{alg_gradient_estimation} to quickly fit the adapter weights in each new model. 
We describe the procedure details in Algorithm \ref{alg_adaboost} in the Appendix. 















\newpage

\begin{algorithm*}[t!]
\raggedright
\caption{{{AdaBoost for Multitask Learning}}}\label{alg_adaboost}
\textbf{Input}: $n$ training sets; A pretrained model $h_{\theta^\star}$\\
\textbf{Require}: Iterations $M$; Number of classes $K$\\
{/*\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad~{\itshape \underline{Constructing one model at each iteration}} \hfill */}
\begin{algorithmic}[1]
\State Initialize the weights $w_i^{(0)}  = \frac{1}{|\cD|}; \text{ for } (s_i, y_i) \in \cD_{\set{1, 2, \dots, n}}$. 
\For{$m = 1, 2, \ldots, M$}
\State Fit a model $h_{\theta^{(m)}}$ to the combined data set of all tasks $\cD$ using weights $w_i^{(m-1)}$, using Algorithm \ref{alg_gradient_estimation}.
\State Compute ${err}^{(m)}$ as
\[
\sum_{i=1}^{|\cD|} w_i^{(m-1)}  \mathbb{1}\big(y_i \neq h_{\theta^{(m)}}(s_i, y_i)\big)/\sum_{i=1}^{|\cD|} w_i^{(m-1)} 
\]
\State Compute 
\[
\alpha^{(m)} = \log \frac{1 - err^{(m)}}{err^{(m)}} + \log(K-1)
\]
\State Update weights
\[
w_i^{(m)}  \leftarrow w_i^{(m-1)} \exp\Big(\alpha^{(m)}\mathbb{1}\big(y_i \neq h_{\theta^{(m)}}(s_i, y_i)\big)\Big)
\]
\State Normalize the weights
\EndFor
\end{algorithmic}
{/*\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad~{\itshape \underline{Ensembling multitask models}} \hfill */}
\begin{algorithmic}[1]
\State Ensemble the models through a weighted average 
\[
h(s, y) = \sum_{m=1}^{M} \alpha^{(m)} h_{\theta^{(m)}}(s, y)
\]
\end{algorithmic}
\end{algorithm*}


\begin{algorithm*}[t!]
\raggedright
\caption{{{Gradient Boosting for Multitask Learning}}}\label{alg_gradient_boost}
\textbf{Input}: $n$ training sets; A pretrained model $h_{\theta^\star}$\\
\textbf{Require}: Iterations $M$; Learning rate $\eta$\\
{/*\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad~{\itshape \underline{Constructing one model at each iteration}} \hfill */}
\begin{algorithmic}[1]
\State Fit an initial model on the combined set of $n$ datasets with original labels, denoted as $h^{(0)} = h_{\theta^{(0)}}$. 
\For{$m = 1, 2, \ldots, M$}
\State Compute the gradient w.r.t. current model predictions, for each sample $(s_i, y_i)$,
\[
r_{i}^{(m)} = - \Big [ \frac{\partial \cL}{\partial h^{(m-1)}(s_i, y_i)} \Big ] = 1 - p_i^{(m-1)}
\]
where $p_i^{(m-1)}$ is the current prediction probability for the correct class label of sample $i$. 
\item Fit a model $h_{\theta^{(m)}}$ to the combined data set of $\set{(s_i, r_i)}_{i=0}^{|\cD|}$, using Algorithm \ref{alg_adaboost}. 
\item Update current ensemble 
\[
h^{(m)} = h^{(m-1)} + \eta h_{\theta^{(m)}}
\]
\EndFor
\end{algorithmic}
{/*\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad~{\itshape \underline{Ensembling multitask models}} \hfill */}
\begin{algorithmic}[1]
\State Return the final ensemble
\[
h(s, y) = h^{(0)}(s, y) + \eta \sum_{m=1}^{M} h_{\theta^{(m)}}(s, y)
\]
\end{algorithmic}
\end{algorithm*}




\section{Experiment Details}


\begin{table}[h!]
\centering
\caption{The average test accuracy of fine-tuning Llama-1.1B on six tasks from SuperGLUE benchmark. We use LoRA as the base fine-tuning procedure. For quantized model, we use QLoRA as the base fine-tuning procedure. We run each experiment with three random seeds.} 
\resizebox{0.5\textwidth}{!}
{
\begin{tabular}{lcccccccc}
\toprule
 & \makecell{Average \\ accuracy (\%)} & \makecell{Training \\ Memory} & \makecell{Inference \\ Memory} \\
\midrule
Naive MTL (16-bit) & 76.46 & 19.5 GB & 4.5 GB \\ 
Naive MTL (4-bit) & 75.14 & 13.0 GB & 1.0 GB \\ 
Naive MTL (3-bit) & 73.23 & 12.7 GB & 0.8 GB\\ 
Naive MTL (2-bit) & 55.26 & 12.5 GB & 0.5 GB\\  \midrule
Model soups & 48.65 & 19.5 GB & 4.5 GB  \\
Task arithmetic  & 62.29 & 19.5 GB & 4.5 GB   \\
TIES & 53.20 & 19.5 GB & 4.5 GB  \\ \midrule
Average ensembling  & 66.06 & 52.2 GB & 9.0 GB\\
Max ensembling & 74.18 & 52.2 GB & 9.0 GB \\  \midrule
Our approach (Algorithm \ref{alg_random_forest}) & \textbf{77.18} & 13.0 GB & 1.4 GB\\ 
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h!]
\centering
\caption{The average test accuracy of fine-tuning Llama-1.1B on six tasks from SuperGLUE benchmark. We use QLoRA for the base fine-tuning procedure. We run each experiment with three random seeds.} 
\resizebox{0.48\textwidth}{!}
{
\begin{tabular}{lcccccccc}
\toprule
Grouped by & $k$ & \makecell{Average \\ accuracy (\%)} & \makecell{Training \\ Memory} & \makecell{Inference \\ Memory} \\
\midrule
Task categories & 4 & 75.59 & 13.0 GB & 1.4 GB \\
Pairwise task affinity & 2 & 76.44 & 13.0 GB & 1.2 GB\\
Pairwise task affinity & 3 & 76.47 & 13.0 GB & 1.3 GB \\
Pairwise task affinity & 4 & 76.80 & 13.0 GB & 1.4 GB \\
Relevance score & 2 & 76.73 & 13.0 GB & 1.2 GB \\
Relevance score & 3 & 77.06 & 13.0 GB & 1.3 GB \\
Relevance score & 4 & \textbf{77.18} & 13.0 GB & 1.4 GB \\ 
\bottomrule
\end{tabular}
}
\end{table}




\begin{table*}[ht!]
\centering
\caption{We evaluate the first-order approximation errors within the fine-tuning region close to the model pre-trained initialization. 
We measure the fine-tuned distance as $\frac{\norm{X-\theta^\star}}{\norm{\theta^\star}}$. We evaluate the RSS
error between $h_X(s, y)$  and the first-order approximation using the pretrained model weights $\theta^\star$.
To ensure the statistical significance of these results, we report the average over $50$ random task subsets.
\DL{Reorganize the table according to Figure 2.}
}\label{tab_approximation_pretrained_models}
{\small\begin{tabular}{@{}cccccccccc@{}}
\toprule
\textbf{Dist.}/RSS & {\textbf{GPT-Neo-125M}} & {\textbf{GPT-Neo-1.3B}} & {\textbf{GPT-Neo-2.7B}} & {\textbf{GPT-Neo-20B}} & {\textbf{Llama-3-1B}} & {\textbf{Llama-3-8B}} \\\midrule
& \multicolumn{6}{c}{Full-precision pretrained model with LoRA}  \\ \midrule
Memory Usage & 6.4GB & 19.6 GB & 31.0 GB & 84.0 GB & 26.4 GB & 43.5 GB \\ \midrule
2\% &   $5.6_{\pm 0.3}\times10^{-5}$  & $4_{\pm 0.1}\times10^{-4}$ &$ 5_{\pm 0.9}\times10^{-4}$ &  $9_{\pm 0.7}\times10^{-5}$ & $6_{\pm 0.5}\times10^{-5}$ &$3_{\pm 0.3}\times10^{-5}$\\
4\% &   $5.7_{\pm 0.2}\times10^{-5}$  & $4_{\pm 0.1}\times10^{-4}$ &$ 8_{\pm 0.5}\times10^{-4}$ & $9_{\pm 0.6}\times10^{-5}$ & $1_{\pm 0.3}\times10^{-4}$ &$6_{\pm 0.9}\times10^{-5}$\\
6\% &   $8.4_{\pm 0.3}\times10^{-5}$ &  $5_{\pm 0.3}\times10^{-4}$ &$ 9_{\pm 0.8}\times10^{-4}$ & $2_{\pm 0.7}\times10^{-4}$ & $3_{\pm 0.7}\times10^{-4}$ &$3_{\pm 0.6}\times10^{-4}$\\
8\% &   $1.2_{\pm 0.6}\times10^{-4}$  & $5_{\pm 0.8}\times10^{-4}$ &$ 2_{\pm 0.3}\times10^{-3}$ & $3_{\pm 0.6}\times10^{-4}$ & $4_{\pm 0.9}\times10^{-4}$ &$4_{\pm 0.4}\times10^{-4}$\\
10\% &   $1.6_{\pm 0.3}\times10^{-4}$ & $5_{\pm 1.2}\times10^{-4}$ &$ 2_{\pm 0.7}\times10^{-3}$ & $5_{\pm 0.3}\times10^{-4}$ & $5_{\pm 0.8}\times10^{-3}$ & $5_{\pm 0.4}\times10^{-4}$\\ \midrule
& \multicolumn{6}{c}{4-bit quantized pretrained model with Quantized LoRA} \\ \midrule
Memory Usage & 5.8 GB & 13.3 GB & 26.6 GB & 42.6 GB & 15.6 GB  & 22.9 GB\\ \midrule
2\% &   $4.6_{\pm 0.1}\times10^{-2}$  & $ 3_{\pm 1.5}\times10^{-3}$ &$2_{\pm 0.0}\times10^{-2}$ & $3_{\pm 0.1}\times10^{-4}$ & $9_{\pm 1.0}\times10^{-3}$ & $1_{\pm 0.3}\times10^{-3}$\\
4\% &   $4.6_{\pm 0.1}\times10^{-2}$  & $ 1_{\pm 0.4}\times10^{-2}$ &$2_{\pm 0.1}\times10^{-2}$ & $3_{\pm 0.2}\times10^{-4}$ & $2_{\pm 0.7}\times10^{-2}$ & $3_{\pm 0.1}\times10^{-3}$\\
6\% &   $4.7_{\pm 0.1}\times10^{-2}$  & $ 2_{\pm 1.0}\times10^{-2}$ &$2_{\pm 0.1}\times10^{-2}$ & $5_{\pm 2.0}\times10^{-4}$ & $6_{\pm 1.1}\times10^{-2}$ & $9_{\pm 0.8}\times10^{-3}$\\
8\% &   $4.8_{\pm 0.2}\times10^{-2}$  & $ 6_{\pm 0.6}\times10^{-2}$ &$2_{\pm 0.1}\times10^{-2}$ & $7_{\pm 0.2}\times10^{-4}$ & $7_{\pm 1.8}\times10^{-2}$ & $1_{\pm 0.2}\times10^{-2}$\\
10\% &  $4.8_{\pm 0.1}\times10^{-2}$  & $ 7_{\pm 1.7}\times10^{-2}$ &$2_{\pm 0.2}\times10^{-2}$ & $8_{\pm 0.8}\times10^{-4}$ & $9_{\pm 0.9}\times10^{-2}$ & $2_{\pm 0.2}\times10^{-2}$ \\ 
\midrule
\textbf{Dist.}/RSS & {\textbf{Llama-3.2-1B}} & {\textbf{Llama-3.2-3B}}  & {\textbf{GPT-J-6B}} & {\textbf{Llama-3-8B}} & & {\textbf{Llama-2-13B}} \\\midrule
& \multicolumn{6}{c}{Full-precision pretrained model with Adapters}  \\ \midrule
Memory Usage & \\ \midrule
2\%   & $8.9_{\pm 3.0}\times10^{-3}$ & $ 2.8_{\pm 1.3}\times10^{-2}$ & $ 1.3_{\pm 0.2}\times10^{-6}$ & $ 3.5_{\pm 0.8}\times10^{-3}$ &  & $ 7.7_{\pm 1.1}\times10^{-7}$\\
4\%   & $1.5_{\pm 1.0}\times10^{-2}$ & $ 3.1_{\pm 1.8}\times10^{-2}$ & $ 1.4_{\pm 0.1}\times10^{-6}$ & $ 2.8_{\pm 1.3}\times10^{-3}$ &  & $ 1.2_{\pm 0.8}\times10^{-6}$\\
6\%   & $2.1_{\pm 1.1}\times10^{-2}$ & $ 4.9_{\pm 2.7}\times10^{-2}$ & $ 1.9_{\pm 0.4}\times10^{-6}$ & $ 3.4_{\pm 0.8}\times10^{-3}$ &  & $ 1.4_{\pm 0.1}\times10^{-6}$\\
8\%   & $2.1_{\pm 0.5}\times10^{-2}$ & $ 5.1_{\pm 0.1}\times10^{-2}$ & $ 2.2_{\pm 1.6}\times10^{-6}$ & $ 4.1_{\pm 0.7}\times10^{-3}$ &  & $ 1.5_{\pm 0.8}\times10^{-6}$\\
10\%  & $7.0_{\pm 1.1}\times10^{-2}$ & $ 7.5_{\pm 6.4}\times10^{-2}$ & $ 2.9_{\pm 1.9}\times10^{-6}$ & $ 6.9_{\pm 6.7}\times10^{-3}$ &  & $ 1.5_{\pm 0.7}\times10^{-6}$\\ \midrule
& \multicolumn{6}{c}{4-bit quantized pretrained model with Quantized adapters} \\ \midrule
Memory Usage & \\ \midrule
2\%   & $7.0_{\pm 1.7}\times10^{-3}$  & $1.5_{\pm 0.2}\times10^{-2}$  & $3.0_{\pm 1.6}\times10^{-6}$  &    &  $ 6.7_{\pm 0.0}\times10^{-7}$  &  $ 1.8_{\pm 0.3}\times10^{-6}$ \\
4\%   & $1.1_{\pm 0.9}\times10^{-2}$  & $1.7_{\pm 0.8}\times10^{-2}$  & $3.1_{\pm 0.8}\times10^{-6}$  &    &  $ 7.3_{\pm 0.8}\times10^{-7}$  &  $ 2.1_{\pm 1.4}\times10^{-6}$ \\
6\%   & $1.1_{\pm 0.9}\times10^{-2}$  & $1.8_{\pm 0.6}\times10^{-2}$  & $5.4_{\pm 3.4}\times10^{-6}$  &    &  $ 8.0_{\pm 0.5}\times10^{-7}$  &  $ 2.2_{\pm 1.8}\times10^{-6}$ \\
8\%   & $2.6_{\pm 3.8}\times10^{-2}$  & $2.2_{\pm 1.3}\times10^{-2}$  & $6.1_{\pm 6.4}\times10^{-6}$  &    &  $ 8.8_{\pm 1.1}\times10^{-7}$  &  $ 1.8_{\pm 0.4}\times10^{-6}$ \\
10\%  & $1.5_{\pm 0.6}\times10^{-2}$  & $4.0_{\pm 1.9}\times10^{-2}$  & $9.1_{\pm 9.6}\times10^{-6}$  &    &  $ 1.1_{\pm 0.2}\times10^{-6}$  &  $ 2.5_{\pm 0.6}\times10^{-6}$ \\ 
\bottomrule
\end{tabular}}
\end{table*}








{}

